Alternative passive maps in the Brayton-Moser framework: Implications on control and optimization

In the recent years, passivity theory has gained renewed attention because of its advantages and practicality in modeling of multi-domain systems and constructive control techniques. Unlike Lyapunov theory, passivity theory takes a behavioral approach in its control design methodologies. Hence, it provides solutions, which not only achieve the control objectives, but are also easily interpretable in the standard engineering parlance. The fundamental idea in passivity based control (PBC) methodologies is to find a controller that renders the closed-loop system passive. It is well known that, the PBC methodologies that rely on power-conjugate port-variables do not work for control objectives that require bounded power and unbounded energy. This is commonly known as the dissipation obstacle. One possible alternative that has been well explored, in the case of finite dimensional systems, is Brayton-Moser formulation. However, designing controllers in this framework leads to various difficulties, such as, solving for partial differential equations and finding storage functions satisfying a gradient structure.

==> Thesis_Passivity.tex <==
\chapter{System theoretic Prerequisites}
 
 
%\section{Passivity}
\section{Port-Hamiltonian (pH) system and Dirac structures}
In general, a port-Hamiltonian system with dissipation, in an n-dimensional state space manifold $\mathcal{X}$ with input space $\mathcal{U}= \mathbb{R}^m$  and output space $\mathcal{Y}= \mathbb{R}^m$ is represented as
\begin{align}\label{PHDS}
\begin{split}
\dot{x}&=\left[J(x)-R(x)\right]\dfrac{\partial H}{\partial x}+g(x) u\\
y&=g^\top (x)\dfrac{\partial H}{\partial x}
\end{split}
\end{align}
where $x\in \mathcal{X}$ is the energy variable and the smooth function $H(x):\mathcal{X}\rightarrow \mathbb{R}$ represents the total energy stored, otherwise called as Hamiltonian and  $u\in \mathcal{U}$, $y\in \mathcal{Y}$ are called input, output port-variables respectively, $m\leq n$. The $n\times n$ matrices $J(x)$ and $R(x)$ satisfies $J(x)=-J^\top (x)$ and $R(x)=R^\top(x)\geq 0$. The input matrix $g(x)\in \mathbb{R}^{n\times m}$ and skew-symmetric matrix $J(x)$ captures the systems interconnection structures, where as, the positive semi-definite matrix $R(x)$ captures the dissipation (or resistive) structure in the system. By the properties of $J(x)$ and $R(x)$, it immediately follows that
\begin{align}\label{dPHDS}
\begin{split}
\dfrac{d}{dt}H(x)&= \dot{x}^\top \dfrac{\partial H}{\partial x}\\
&= \left(\left[J(x)-R(x)\right]\dfrac{\partial H}{\partial x}+g(x) u\right)^\top \dfrac{\partial H}{\partial x}\\
&= -\dfrac{\partial H}{\partial x}^\top R(x)\dfrac{\partial H}{\partial x}+u^\top g^\top \dfrac{\partial H}{\partial x}\\
&\leq u^\top y
\end{split}
\end{align}
%\beqn
%\dfrac{d}{dt}H(x)&=& \dot{x}^\top \dfrac{\partial H}{\partial x}\\
%&=& \left(\left[J(x)-R(x)\right]\dfrac{\partial H}{\partial x}+g(x) u\right)^\top \dfrac{\partial H}{\partial x}\\
%&=& -\dfrac{\partial H}{\partial x}^\top R(x)\dfrac{\partial H}{\partial x}+u^\top g^\top \dfrac{\partial H}{\partial x}\\
%&\leq& u^\top y
%\eeqn
This implies that the pH system \eqref{PHDS} is passive with port-variables $u$ and $y$. As the Hamiltonian $H$ represents the total energy stored in the system, $\dot{H}$ represents the instantaneous power transfer. Moreover, $u$ and $y$ are called power-conjugate port-variables, meaning, their product $u^\top y$ represents the power flow between the environment and the system. Well-known examples of such pairs are voltage-current in electrical circuits and force-velocity in mechanical systems. Consequently, the equation \eqref{dPHDS} gives the {\em dissipative} inequality
\begin{align}\label{iPHDS}
\begin{split}
\underbrace{H(x(t_1)-H(x(t_0)))}_{\text{\large Stored\;\;energy}}&=  \underbrace{-\int_{t_0}^{t_1}\left(\dfrac{\partial H}{\partial x}^\top R(x)\dfrac{\partial H}{\partial x}\right)dt}_{\text{\large Dissipated energy}}+ \underbrace{\int_{t_0}^{t_1}u^\top ydt}_{\text{\large Supplied energy }}
\end{split}
\end{align}
where $t_0\leq t_1$ and $H$, $u^\top y$ represents the storage function and the supply rate respectively.
\subsection*{Dirac Structures}
In network theory, the Tellegen theorem states that the summation of instantaneous power in all the branches of the network is zero. Dirac structure generalizes the underlying geometric structure of Tellegen theorem (power conservation). Let $\mathcal{F}\times \mathcal{F}^\ast$ space of these power variable, where the linear space $\mathcal{F}$ is called flow space and $\mathcal{E}=\mathcal{F}^\ast$ is the dual space of $\mathcal{F}$, called as effort space. In the case of network theory, these spaces can be interpreted as spaces of branch voltages and currents, vice-versa (in the case of mechanical systems they represents generalized forces and generalized velocities). Let $f\in \mathcal{F}$ and $e\in \mathcal{E}$ denotes the flow and effort variables respectively. The power in the total space of port variables ($\mathcal{F}\times \mathcal{E}$) can be defined as 
\beq
P=\left<e|f\right>,\;\; (f,e)\in\mathcal{F}\times \mathcal{E}
\eeq
where $\left<e|f\right>$ denotes the duality product, that is, the linear functional $e\in \mathcal{E}$ acting on $\mathcal{F}$. In the case of $\mathcal{F}=\mathbb{R}^m$ 
\beqn
\left<e|f\right>&=&e^\top f
\eeqn
that is, the duality product can be identified with the inner-product defined on $\mathbb{R}^m$. 
\begin{definition}\cite{van2014port}
	Consider a finite-dimensional linear space $\mathcal{F}$ with $\mathcal{E}=\mathcal{F}^\ast$. A subspace $D\subset \mathcal{F}\times \mathcal{E}$ is a (constant) Dirac structure if
	\begin{itemize}
		\item [1.]$\left<e|f\right>=0$, for all $(f,e)\in \mathcal{D}$ \;\;\;\; (Power conservation)
		\item[2.]dim $\mathcal{D}$=dim $\mathcal{F}$\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; (maximal dimension of subspace $\mathcal{D}$ )
	\end{itemize}
\end{definition}
Next, we present an equivalent definition for the Dirac structure, which will be useful in presenting the Dirac formulation of infinite dimensional systems in Chapter 5.

\begin{definition}
	A (constant) Dirac structure on $\mathcal{F}\times \mathcal{E}$ is a subspace $\mathcal{D}\subset \mathcal{F}\times \mathcal{E}$ such that 
	\beq
	\mathcal{D}&=&\mathcal{D}^{\perp}
	\eeq
	where $\perp$ denotes the orthogonal complement with respect to the bilinear form $\left<\left<\;,\right>\right>$ given as
	\beq
	\left<\left<(f^a,e^a),(f^b,e^b)\right>\right>&=&\left<e^a,f^b\right>+\left<e^b,f^a\right>, \;\;\;\;(f^a,e^a),(f^b,e^b)\in \mathcal{F}\times \mathcal{E}
	\eeq
	or equivalently
	\beq
	D^{\perp}:=\left\{\left(f^a,e^a\right)|\left<\left<(f^a,e^a),(f,e)\right>\right>=0,(f,e)\in \mathcal{D}\right\}
	\eeq
\end{definition}
For further exposition on Dirac structures and their alternate representation see \cite{van2014port,l2gain, courant1990dirac, dorfman1993dirac,dalsmo1998representations}.
%The smooth function $H(x):\mathcal{X}\rightarrow \mathbb{R}$ represents the total energy stored, otherwise called as Hamiltonian.
\section{Control by inter connection}
In control by interconnection, we assume that the controller is a port-Hamiltonian system with dissipation (a dynamical system usually implemented on a computer) 
\begin{align}\label{cPHDS}
\begin{split}
\dot{x}_c&=\left[J(x_c)-R(x_c)\right]\dfrac{\partial H_c}{\partial x_c}+g_c(x_c) u_c\\
y_c&=g_c^\top (x_c)\dfrac{\partial H_c}{\partial x_c}
\end{split}
\end{align}
interconnected to the physical system \eqref{PHDS} using a standard feedback interconnection
\beqn
\begin{matrix}
	u=-y_c+v&u_c=y+v_c
\end{matrix}
\eeqn
such that the closed loop system
\begin{align}\label{cibPHDS}
\begin{split}
\begin{bmatrix}
\dot{x}\\
\dot{x}_c
\end{bmatrix}&=\begin{bmatrix}
J(x)-R(x) &-g(x)g_c^\top (x_c)\\g_c(x_c)g^\top &J(x_c)-R(x_c)
\end{bmatrix}\begin{bmatrix}
\dfrac{\partial H}{\partial x}\\\dfrac{\partial H_c}{\partial x_c}
\end{bmatrix}+\begin{bmatrix}
g(x)&0\\0&g_c(x_c)
\end{bmatrix}\begin{bmatrix}
v\\v_c
\end{bmatrix}\\
\begin{bmatrix}
y\\y_c
\end{bmatrix}&=\begin{bmatrix}
g(x) &0\\0&g_c(x_c)
\end{bmatrix}^\top\begin{bmatrix}
\dfrac{\partial H}{\partial x}\\\dfrac{\partial H_c}{\partial x_c}
\end{bmatrix}
\end{split}
\end{align}
is again a port Hamiltonian system with dissipation. Next, we find the invariant functions called Casimir's $\mathcal{C}(x,x_c)$, that are independent of the closed-loop Hamiltonian $H(x)+H_c(x_c)$, using
\begin{align}\label{casPHDS}
\begin{split}
\begin{bmatrix}
\dfrac{\partial \mathcal{C}}{\partial x}\\\dfrac{\partial \mathcal{C}}{\partial x_c}
\end{bmatrix}^\top\begin{bmatrix}
J(x)-R(x) &-g(x)g_c^\top (x_c)\\g_c(x_c)g^\top &J(x_c)-R(x_c)
\end{bmatrix}&=0.
\end{split}
\end{align}
These Casimir's, that relate the plant state to controller state, are used to shape the closed-loop Hamiltonian  at the desired operating point by replacing $H(x)+H_c(x_c)$ by $H(x)+H_c(x_c)+H_a(\mathcal{C})$. Further, if the Casimir's are of the form 
\beq \label{cas::clp_inv} \mathcal{C}(x,x_c)=x_c-C(x)\eeq
then we can eliminate $x_c$ from  \eqref{cibPHDS} by restricting the closed-loop dynamics to the level set $L=\left\{(x,x_c)|x_c=C(x)\right\}$. There by, we can use  $H(x)+H_c(C(x))$ as the new storage function. The main disadvantage of this methodology is that the Casimir's of the form \eqref{cas::clp_inv} exist if and only if $C(x)$ satisfies
\beq
\dfrac{\partial C}{\partial x}^\top J(x)\dfrac{\partial C}{\partial x}&=&J_c(x_c)\\
R(x)\dfrac{\partial C}{\partial x}&=& 0\label{cas::diss_obs}\\
R_c(x_c)&=&0\\
\dfrac{\partial C}{\partial x}^\top J(x)&=&g_c(x_c)g(x)^\top
\eeq
\section{Dissipation Obstacle}
In standard control by interconnection methodologies \citep{OrtVanCasAst}, we assume that both plant and controller \kcn{are} passive. Plants that extract infinite energy at nonzero equilibrium, cannot be stabilized under this assumption. %(as shown below in Example \ref{moti::example_pRLC})
 This can also be seen from equation \eqref{cas::diss_obs}. If there exists a dissipative element $R(x_i)\neq 0$ at some state  $x_i$ ($x_i$ denotes $i^{th}$ coordinate of state vector $x$, that need to be shaped), then from equation, \eqref{cas::diss_obs} $R(x_i)\dfrac{\partial C}{\partial x_i}=0\implies \dfrac{\partial C}{\partial x_i}=0$. This implies the achievable Casimir is independent of $x_i$, hence $x_i$ cannot be shaped. A port-Hamiltonian system is said to be stymied with {\em dissipation obstacle}, if it extracts infinite energy at nonzero equilibrium or equivalently if it has non-zero dissipation at the coordinate that requires shaping \citep{ortega2001putting}. This is a common phenomenon in finite dimensional RLC circuits. We now present an example using a parallel RLC circuit (Figure \ref{fig:pRLC}).
%\subsection{Finite-dimensional pH systems: Example of parallel RLC circuit}
\begin{example}\label{moti::example_pRLC}
	\begin{figure}[h]
		\centering
		\includegraphics[width=0.6\linewidth]{pRLC}
		\caption{Parallel RLC circuit}
		\label{fig:pRLC}
	\end{figure}
	Consider the parallel RLC circuit (as shown in Figure \ref{fig:pRLC}) with voltage $v_C$ across the capacitor $C$ and current $i_L$ through the inductor $L$ as the state variables. The dynamics of this system are:
	\beq \label{moti::pRLC_eqn}
	\begin{matrix}
		-L\dfrac{di_L}{dt}&=& R_Li_L+v_C-V_s\\C\dfrac{dv_C}{dt}&=&i_L-\dfrac{v_C}{R_C}
	\end{matrix}
	\eeq
	where $R_L$ is the series resistance of the inductor $L$, $R_C$ is the parallel resistance of the capacitor $C$ and $V_s$ is the voltage source. It can be shown that this system is passive with total energy
	\beqn
	E=\dfrac{1}{2}Li^2_L+\dfrac{1}{2}Cv_C^2
	\eeqn
	as storage function and port variables being input $V_s$ and output $i_L$, i.e. $\dot E\leq V_si_L$. Further at a non zero operating point $(i_L^\ast,v_C^\ast)$, we have a non zero supply rate $V_s^\ast i_L^\ast\neq 0$. This implies \kcn{that at} equilibrium, system extracts infinite energy from the controller (or the controller have to supply infinite energy to the plant), thus proving the existence of {\em dissipation obstacle}. 
	Next we show the existence of {\em dissipation obstacle} in infinite-dimensional systems, using transmission line system (with non zero boundary conditions) as an example. 
\end{example}


% \subsection{Infinite-dimensional pH systems: Example of an Transmission line system with non zero boundary}
% \begin{example}\label{moti::example_TL}
% 	Let $0<z<1$ represent the spatial domain of the transmission line with $L$, $C$, $R$ and $G$ denoting the specific inductance, capacitance, resistance, and conductance respectively. We further assume that these are independent of the spatial variable $z$. Denote $i(z,t)$ and $v(z,t)$ as the line current and line voltage of transmission line system. Consider the transmission line system (modeled using telegraphers equations) interconnected to boundary as shown in Figure \ref{fig::abc}. The dynamics of this system are
% 	\begin{figure}%[h]
% 		\begin{center}
% 			\includegraphics[scale=.5]{TL} \caption{Transmission line system} \label{fig::abc}
% 		\end{center}
% 	\end{figure}
% 	\begin{align}
% 	\begin{matrix}
% 	-Li_t&=& v_z+Ri\\
% 	Cv_t&=& -Gv-i_z
% 	\end{matrix}\hspace{8mm}0<z<1\label{telegraphers}\\
% 	\begin{matrix}
% 	I_0&=& C_0v_{0t}+i_0\\
% 	v_0	&=& v_{C_0}-i_0R_0
% 	\end{matrix}\hspace{13mm}z=0\label{z0}\\
% 	\begin{matrix}
% 	i_1&=& C_1v_{C_1t}\\
% 	v_1&=& R_1i_1+v_{C_1}
% 	\end{matrix}\hspace{12mm}z=1.\label{z1}
% 	\end{align}
% 	where $v_{C0}$ and $v_{C1}$ denote voltages across the capacitors $C_0$ and $C_1$ respectively and  $I_0$ represents the current source at $z=0$. Additionally, the boundary voltages and currents are denoted by $v_0=v(0,t)$, $i_0=i(0,t)$, $v_1=v(1,t)$ and $i_1=i(1,t)$.
% \end{example}

% \begin{proposition}\label{prop::dissp}
% 	The transmission line system described by the equations \eqref{telegraphers}, \eqref{z0} and \eqref{z1} cannot be stabilized \kcn{at} any non trivial equilibrium point with passive maps obtained by using the total energy given by
% 	\beq\label{moti::energy}
% 	E=\dfrac{1}{2}\int_{0}^{1}\left(Li^2+Cv^2\right)dz+\dfrac{1}{2}C_0v_{c_0}^2+\dfrac{1}{2}C_1v_{c_1}^2.
% 	\eeq
% 	as the storage function.
% \end{proposition}
% \begin{proof}Differentiating \eqref{moti::energy} and using \eqref{telegraphers}, \eqref{z0} and \eqref{z1}; we arrive at the following inequality
% 	\beq\label{mot_pmaps}
% 	\dot E \leq I_0 v_{C_0}.
% 	\eeq
% 	{\em Equilibrium points:}

% 	{\em At equilibrium, equations \eqref{telegraphers}, \eqref{z0} and \eqref{z1} evaluate to
% 		\begin{align}
% 		\begin{matrix}
% 		i^\ast_z +Gv^\ast&=&0, \hspace{2mm}& Ri^\ast +v^\ast_z&=&0
% 		\end{matrix}\hspace{10mm}0<z<1\label{eq_telegraphers}\\
% 		\begin{matrix}
% 		I_0^\ast &=& i_0^\ast, \hspace{2mm} & v_0^\ast	&=& v_{C_0}^\ast-i_0^\ast R_0
% 		\end{matrix}\hspace{11mm}z=0\label{eq_z0}\\
% 		\begin{matrix}
% 		i_1^\ast &=& 0, \hspace{2mm} & v_1^\ast&=& v_{C_1}^\ast
% 		\end{matrix}\hspace{12mm}z=1.\label{eq_z1}
% 		\end{align}
% 		Finally, solving partial differential equation \eqref{eq_telegraphers} using the boundary conditions \eqref{eq_z0} and \eqref{eq_z1}, the solution for $i^\ast(z), v^\ast(z)$ takes the form
% 		\beq
% 		\begin{matrix}\label{sol_trans_eq}
% 			i^\ast(z)=\dfrac{G}{\omega}v_{C_1}^\ast \sinh(\omega (1-z)), &
% 			v^\ast(z)= v_{C_1}^\ast \cosh(\omega (1-z)
% 		\end{matrix}
% 		\eeq
% 		where $\omega =\sqrt{RG}$.
% 		Using equations \eqref{eq_z0}, \eqref{eq_z1} and \eqref{sol_trans_eq} it can be shown that the supply rate $I_0^\ast v_{C_0}^\ast  \neq 0$ at equilibrium. This proves the existence of dissipation obstacle \citep*{OrtVanMas}.} %\kcn{For a brief overview on dissipation obstacle in the case of transmissionline system we refer to \citep{AleCla}.}
% \end{proof}
% This problem can be prevented either by relaxing the assumption that controller has to be passive \citep{KoopDim} or by finding new passive maps \citep{ElosiaDimOrt}. In this note we make use of the latter. 
% It can be seen from \eqref{mot_pmaps} that \kcn{``adding a differentiation"} on the output port variable obviates the {\em dissipation obstacle}. One alternative is to search for new passive maps within the Brayton Moser framework. 
% %This motivated our search for new passive maps that eliminates dissipation obstacle.
% In the next section we will briefly outline the BM formulation of finite dimensional circuits and present the new passive map using parallel RLC circuit in Example \ref{moti::example_pRLC}.

==> Thesis_to_do.tex <==
\chapter{Todo}
\begin{enumerate}
    \item[1] Give a generic formulation of dissipation obstacle. And write the Alasandros mistake in dissipation obstacle section
    \item[2] Try and prove $\tilde{A}$ is negative definite in generic formulation.
    \item[3] Add a different example for primal-dual optimization algorithm.
    \item [4] Zero-state detectability
    \item [5] Passivity based control ---Energy shaping.. like finding a potential function and all...make the closed loop system passive.. EB-PBC, IDA PBC(IDA PBC is more general and avoids dissipation obstacle)
    \item[6] Control by inter connection... inter connect two dynamical system to make the closed loop system passive..Casimirs come here
\end{enumerate}
Chapter-2
\begin{enumerate} 
\item Port-Hamiltonian systems and Dirac structures
\item Energy Shaping and dissipation obstacle
\item Energy to co-energy formulation

\item Infinite-dimensional port Hamiltonian systems
\item Stability in Infinite dimensional systems
\item Energy shaping and dissipation obstacle for inifite-dime sys..Alasandros paper?
\item Discussion of 1964-paper?
\item Brayton-Moser formulation and Dirac structures (Concentrate on Blankinestien paper)
\item Infinite dimensional sytems intro (chapter)
\item Alaternative passive maps for infinite dimensional systems ..introduction missing
\end{enumerate}
chapter-3
\begin{enumerate}
\item We have to give some material on contraction Mapping
\item 
\end{enumerate}

==> ref.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Venkatesh at 2015-09-29 10:33:09 -0500


%% Saved with string encoding Unicode (UTF-8)
@article{mehra2017control,
	title={Control of a class of underactuated mechanical systems obviating matching conditions},
	author={Mehra, Rachit and Satpute, Sumeet G and Kazi, Faruk and Singh, NM},
	journal={Automatica},
	volume={86},
	pages={98--103},
	year={2017},
	publisher={Elsevier}
}
@article{stegink2017unifying,
	title={A unifying energy-based approach to stability of power grids with market dynamics},
	author={Stegink, Tjerk and De Persis, Claudio and van der Schaft, Arjan},
	journal={IEEE Transactions on Automatic Control},
	volume={62},
	number={6},
	pages={2612--2622},
	year={2017},
	publisher={IEEE}
}
@article{Guido,
	title={Geometric modeling of nonlinear {RLC} circuits},
	author={Blankenstein, Guido},
	journal={IEEE Transactions on Circuits and Systems I: Regular Papers},
	volume={52},
	number={2},
	pages={396--404},
	year={2005},
	publisher={IEEE}
}
@article{stokes,
	title={{H}amiltonian formulation of distributed-parameter systems with boundary energy flow},
	author={van der Schaft, Arjan J and Maschke, BM},
	journal={Journal of Geometry and Physics},
	volume={42},
	number={1},
	pages={166--194},
	year={2002},
	publisher={Elsevier}
}



@article{pavlov2008incremental,
  title={Incremental passivity and output regulation},
  author={Pavlov, Alexey and Marconi, Lorenzo},
  journal={Systems \& Control Letters},
  volume={57},
  number={5},
  pages={400--409},
  year={2008},
  publisher={Elsevier}
}
@article{kosaraju2018stability,
  title={Stability Analysis of Constrained Optimization Dynamics via Passivity Techniques},
  author={Kosaraju, KC and Chinde, V and Pasumarthy, R and Kelkar, A and Singh, NM},
  journal={IEEE Control Systems Letters},
  volume={2},
  number={1},
  pages={91--96},
  year={2018},
  publisher={IEEE}
}
@book{nijmeijer1990nonlinear,
  title={Nonlinear dynamical control systems},
  author={Nijmeijer, Henk and Van der Schaft, Arjan},
  volume={175},
  year={1990},
  publisher={Springer}
}
@article{angeli2002lyapunov,
  title={A Lyapunov approach to incremental stability properties},
  author={Angeli, David},
  journal={IEEE Transactions on Automatic Control},
  volume={47},
  number={3},
  pages={410--421},
  year={2002},
  publisher={IEEE}
}
@article{fox2013population,
  title={Population games, stable games, and passivity},
  author={Fox, Michael J and Shamma, Jeff S},
  journal={Games},
  volume={4},
  number={4},
  pages={561--583},
  year={2013},
  publisher={Multidisciplinary Digital Publishing Institute}
}
@article{forni2014differential,
  title={A differential Lyapunov framework for contraction analysis},
  author={Forni, Fulvio and Sepulchre, Rodolphe},
  journal={IEEE Transactions on Automatic Control},
  volume={59},
  number={3},
  pages={614--628},
  year={2014},
  publisher={IEEE}
}
@article{cortes2005characterization,
  title={Characterization of gradient control systems},
  author={Cort{\'e}s, Jorge and Van Der Schaft, Arjan and Crouch, Peter E},
  journal={SIAM journal on control and optimization},
  volume={44},
  number={4},
  pages={1192--1214},
  year={2005},
  publisher={SIAM}
}
@inproceedings{forni2013differential,
  title={On differential passivity of physical systems},
  author={Forni, Fulvio and Sepulchre, Rodolphe and Van Der Schaft, AJ},
  booktitle={Decision and Control (CDC), 2013 IEEE 52nd Annual Conference on},
  pages={6580--6585},
  year={2013},
  organization={IEEE}
}
@book{crouch1987variational,
  title={Variational and Hamiltonian control systems},
  author={Crouch, P E and Van der Schaft, Arjan J},
  year={1987},
  publisher={Springer-Verlag New York, Inc.}
}
@article{van2013differential,
  title={On differential passivity},
  author={van der Schaft, Arjan J},
  journal={IFAC Proceedings Volumes},
  volume={46},
  number={23},
  pages={21--25},
  year={2013},
  publisher={Elsevier}
}
@book{hahn1967stability,
  title={Stability of motion},
  author={Hahn, Wolfgang},
  volume={138},
  year={1967},
  publisher={Springer}
}
@book{krasovskiicertain,
  title={Certain Problems of the Theory of Stability of Motion [in Russian], Fizmatgiz, Moscow},
  author={Krasovskii, NN},
  year={1959},
  publisher={English translation by Stanford University Press, 1963}
}

@article{lohmiller1998contraction,
  title={On contraction analysis for non-linear systems},
  author={Lohmiller, Winfried and Slotine, Jean-Jacques E},
  journal={Automatica},
  volume={34},
  number={6},
  pages={683--696},
  year={1998},
  publisher={Elsevier}
}
@article{jeltsema2003passivity,
  title={On passivity and power-balance inequalities of nonlinear RLC circuits},
  author={Jeltsema, Dimitri and Ortega, Romeo and Scherpen, Jacquelien MA},
  journal={IEEE Transactions on Circuits and Systems I: Fundamental Theory and Applications},
  volume={50},
  number={9},
  pages={1174--1179},
  year={2003},
  publisher={IEEE}
}
@article{css_arxiv,
  title={Stability Analysis of Constrained OptimizationProblem Using Passivity Approach},
  author={Kosaraju, KC and Chinde, V and Pasumarthy, R and Kelkar, Atul and Singh, NM},
  archivePrefix = "arXiv",
  journal={arXiv:1708.03212 },
  year={2017},
}
@article{BMnetworks,
  title={A theory of nonlinear networks. I},
  author={Brayton, RK and Moser, JK},
  journal={Quarterly of Applied Mathematics},
  volume={22},
  number={1},
  pages={1--33},
  year={1964}
}
@book{ben2001lectures,
  title={Lectures on modern convex optimization: analysis, algorithms, and engineering applications},
  author={Ben-Tal, Aharon and Nemirovski, Arkadi},
  year={2001},
  publisher={SIAM}
}
@book{ibaraki1988resource,
  title={Resource allocation problems: algorithmic approaches},
  author={Ibaraki, Toshihide and Katoh, Naoki},
  year={1988},
  publisher={MIT press}
}
@article{xiao2006optimal,
  title={Optimal scaling of a gradient method for distributed resource allocation},
  author={Xiao, Lin and Boyd, Stephen},
  journal={Journal of optimization theory and applications},
  volume={129},
  number={3},
  pages={469--488},
  year={2006},
  publisher={Springer}
}
@article{kelly1998rate,
  title={Rate control for communication networks: shadow prices, proportional fairness and stability},
  author={Kelly, Frank P and Maulloo, Aman K and Tan, David KH},
  journal={Journal of the Operational Research society},
  volume={49},
  number={3},
  pages={237--252},
  year={1998},
  publisher={Springer}
}
@inproceedings{wang2011control,
  title={A control perspective for centralized and distributed convex optimization},
  author={Wang, Jing and Elia, Nicola},
  booktitle={Decision and Control and European Control Conference (CDC-ECC), 2011 50th IEEE Conference on},
  pages={3800--3805},
  year={2011}
}
@article{arrow1958studies,
  title={Studies in linear and non-linear programming},
  author={Arrow, Kenneth Joseph and Hurwicz, Leonid and Uzawa, Hirofumi and Chenery, Hollis Burnley},
  year={1958},
  publisher={Stanford University Press}
}
@article{kose1956solutions,
  title={Solutions of saddle value problems by differential equations},
  author={Kose, T},
  journal={Econometrica, Journal of the Econometric Society},
  pages={59--70},
  year={1956},
  publisher={JSTOR}
}
@inproceedings{bloch1992geometry,
  title={On the geometry of saddle point algorithms},
  author={Bloch, Anthony M and Brockett, Roger W and Ratiu, Tudor S},
  booktitle={Decision and Control, 1992., Proceedings of the 31st IEEE Conference on},
  pages={1482--1487},
  year={1992}
}
@inproceedings{simpson2016input,
  title={Input/output analysis of primal-dual gradient algorithms},
  author={Simpson-Porco, John W},
  booktitle={Communication, Control, and Computing (Allerton), 54th Annual Allerton Conference on},
  pages={219--224},
  year={2016}
}
@article{zhao2006notion,
	title={A notion of passivity for switched systems with state-dependent switching},
	author={Zhao, Jun and Hill, David J},
	journal={Journal of control theory and applications},
	volume={4},
	number={1},
	pages={70--75},
	year={2006},
	publisher={Springer}
}
@article{ortega2003power,
  title={Power shaping: A new paradigm for stabilization of nonlinear RLC circuits},
  author={Ortega, Romeo and Jeltsema, Dimitri and Scherpen, Jacquelien MA},
  journal={IEEE Transactions on Automatic Control},
  volume={48},
  number={10},
  pages={1762--1767},
  year={2003},
  publisher={IEEE}
}
@inproceedings{belk2016stability,
  title={Stability and control of ad hoc dc microgrids},
  author={Belk, Julia A and Inam, Wardah and Perreault, David J and Turitsyn, Konstantin},
  booktitle={Decision and Control (CDC), 2016 IEEE 55th Conference on},
  pages={3271--3278},
  year={2016}
}
@article{lygeros2003dynamical,
  title={Dynamical properties of hybrid automata},
  author={Lygeros, John and Johansson, Karl Henrik and Simic, Slobodan N and Zhang, Jun and Sastry, Shankar S},
  journal={IEEE Transactions on automatic control},
  volume={48},
  number={1},
  pages={2--17},
  year={2003},
  publisher={IEEE}
}
@incollection{l2gain,
  title={$L_2$-gain and passivity techniques in nonlinear control},
  author={Arjan J van der Schaft},
  year={2000},
  publisher={Springer, London}
}
@article{ICCvdotidot,
  title={Control using new passivity property with differentiation at both ports},
  author={Kosaraju, KC and  Pasumarthy, R and Singh, NM and Fradkov, AL},
  journal={Indian Control Conference (ICC)},
  pages={7--11},
  year={2017},
  publisher={IEEE}
}
@article{HybridPassive,
  title={A notion of passivity for hybrid systems},
  author={Zefran, M and  Bullo, F and Stein, M},
  journal={IEEE Conference on Decision and Control (CDC)},
  year={2001}
}
@article{van2011relation,
  title={On the relation between port-Hamiltonian and gradient systems},
  author={van der Schaft, Arjan J},
  journal={IFAC Proceedings Volumes},
  volume={44},
  number={1},
  pages={3321--3326},
  year={2011},
  publisher={Elsevier}
}
@techreport{zavala2011next,
  title={Next-generation building energy management systems and implications for electricity markets.},
  author={Zavala, VM and Thomas, C and Zimmerman, M and Ott, A and others},
  year={2011},
  institution={Argonne National Laboratory (ANL)}
}
@article{cherukuri2016asymptotic,
  title={Asymptotic convergence of constrained primal--dual dynamics},
  author={Cherukuri, Ashish and Mallada, Enrique and Cort{\'e}s, Jorge},
  journal={Systems \& Control Letters},
  volume={87},
  pages={10--15},
  year={2016},
  publisher={Elsevier}
}
@article{yi2015distributed,
  title={Distributed gradient algorithm for constrained optimization with application to load sharing in power systems},
  author={Yi, Peng and Hong, Yiguang and Liu, Feng},
  journal={Systems \& Control Letters},
  volume={83},
  pages={45--52},
  year={2015},
  publisher={Elsevier}
}
@article{roozbehani2012volatility,
  title={Volatility of power grids under real-time pricing},
  author={Roozbehani, Mardavij and Dahleh, Munther A and Mitter, Sanjoy K},
  journal={IEEE Transactions on Power Systems},
  volume={27},
  number={4},
  pages={1926--1940},
  year={2012},
  publisher={IEEE}
}

@article{feijer2010stability,
  title={Stability of primal--dual gradient dynamics and applications to network optimization},
  author={Feijer, Diego and Paganini, Fernando},
  journal={Automatica},
  volume={46},
  number={12},
  pages={1974--1981},
  year={2010},
  publisher={Elsevier}
}
@article{palensky2011demand,
  title={Demand side management: Demand response, intelligent energy systems, and smart loads},
  author={Palensky, Peter and Dietrich, Dietmar},
  journal={IEEE transactions on industrial informatics},
  volume={7},
  number={3},
  pages={381--388},
  year={2011},
  publisher={IEEE}
}
@article{hobbs1992nonlinear,
  title={A nonlinear bilevel model for analysis of electric utility demand-side planning issues},
  author={Hobbs, Benjamin F and Nelson, Sushil K},
  journal={Annals of Operations Research},
  volume={34},
  number={1},
  pages={255--274},
  year={1992},
  publisher={Springer}
}
@article{chen2012real,
  title={Real-time price-based demand response management for residential appliances via stochastic optimization and robust optimization},
  author={Chen, Zhi and Wu, Lei and Fu, Yong},
  journal={IEEE Transactions on Smart Grid},
  volume={3},
  number={4},
  pages={1822--1831},
  year={2012},
  publisher={IEEE}
}
@inproceedings{maasoumy2014model,
  title={Model predictive control approach to online computation of demand-side flexibility of commercial buildings hvac systems for supply following},
  author={Maasoumy, Mehdi and Rosenberg, Catherine and Sangiovanni-Vincentelli, Alberto and Callaway, Duncan S},
  booktitle={American Control Conference (ACC), 2014},
  pages={1082--1089},
  year={2014}
}
@article{mathieu2013state,
  title={State estimation and control of electric loads to manage real-time energy imbalance},
  author={Mathieu, Johanna L and Koch, Stephan and Callaway, Duncan S},
  journal={IEEE Transactions on Power Systems},
  volume={28},
  number={1},
  pages={430--440},
  year={2013},
  publisher={IEEE}
}
@incollection{chen2012optimal,
  title={Optimal demand response: Problem formulation and deterministic case},
  author={Chen, Lijun and Li, Na and Jiang, Libin and Low, Steven H},
  booktitle={Control and optimization methods for electric smart grids},
  pages={63--85},
  year={2012},
  publisher={Springer}
}
@article{henze2003predictive,
  title={Predictive optimal control of active and passive building thermal storage inventory},
  author={Henze, Gregor P and Krarti, Moncef},
  journal={Architectural Engineering--Faculty Publications},
  pages={1},
  year={2003}
}
@article{hamalainen2000cooperative,
  title={Cooperative consumers in a deregulated electricity market—dynamic consumption strategies and price coordination},
  author={H{\"a}m{\"a}l{\"a}inen, Raimo P and M{\"a}ntysaari, Juha and Ruusunen, Jukka and Pineau, Pierre-Olivier},
  journal={Energy},
  volume={25},
  number={9},
  pages={857--875},
  year={2000},
  publisher={Elsevier}
}
@inproceedings{hao2013ancillary,
  title={Ancillary service for the grid via control of commercial building HVAC systems},
  author={Hao, He and Kowli, Anupama and Lin, Yashen and Barooah, Prabir and Meyn, Sean},
  booktitle={American Control Conference (ACC), 2013},
  pages={467--472},
  year={2013}
}
@article{chu1993scheduling,
  title={Scheduling of direct load control to minimize load reduction for a utility suffering from generation shortage},
  author={Chu, Wen-Chen and Chen, Bin-Kwie and Fu, Chun-Kuei},
  journal={IEEE Transactions on Power Systems},
  volume={8},
  number={4},
  pages={1525--1530},
  year={1993},
  publisher={IEEE}
}
@inproceedings{cezar2015stability,
  title={Stability of interconnected DC converters},
  author={Cezar, Gustavo and Rajagopal, Ram and Zhang, Baosen},
  booktitle={Decision and Control (CDC), 2015 IEEE 54th Annual Conference on},
  pages={9--14},
  year={2015}
}
@inproceedings{belk2016stability,
  title={Stability and control of ad hoc dc microgrids},
  author={Belk, Julia A and Inam, Wardah and Perreault, David J and Turitsyn, Konstantin},
  booktitle={Decision and Control (CDC), 2016 IEEE 55th Conference on},
  pages={3271--3278},
  year={2016}
}
@article{khalil1996noninear,
  title={Noninear Systems},
  author={Khalil, Hassan K},
  journal={Prentice-Hall, New Jersey},
  volume={2},
  number={5},
  year={1996}
}
@book{ortega2013passivity,
  title={Passivity-based control of Euler-Lagrange systems: mechanical, electrical and electromechanical applications},
  author={Ortega, Romeo and Perez, Julio Antonio Lor{\'\i}a and Nicklasson, Per Johan and Sira-Ramirez, Hebertt},
  year={2013},
  publisher={Springer Science \& Business Media}
}
@article{emadi2006constant,
  title={Constant power loads and negative impedance instability in automotive systems: definition, modeling, stability, and control of power electronic converters and motor drives},
  author={Emadi, Ali and Khaligh, Alireza and Rivetta, Claudio H and Williamson, Geoffrey A},
  journal={IEEE Transactions on Vehicular Technology},
  volume={55},
  number={4},
  pages={1112--1125},
  year={2006},
  publisher={IEEE}
}
@article{KCoptstab, 
author={K. C. Kosaraju and V. Chinde and R. Pasumarthy and A. Kelkar and N. M. Singh}, 
journal={IEEE Control Systems Letters}, 
title={Stability Analysis of Constrained Optimization Dynamics via Passivity Techniques}, 
year={2017}, 
volume={PP}, 
number={99}, 
pages={1-6}, 
publisher={IEEE}
}
@article{brayton1964some,
  title={Some results on the stability of nonlinear networks containing negative resistances},
  author={Brayton, R and Moser, J},
  journal={IEEE Transactions on Circuit Theory},
  volume={11},
  number={1},
  pages={165--167},
  year={1964},
  publisher={IEEE}
}
@article{jeltsema2004energy,
  title={An energy-balancing perspective of interconnection and damping assignment control of nonlinear systems},
  author={Jeltsema, Dimitri and Ortega, Romeo and Scherpen, Jacquelien MA},
  journal={Automatica},
  volume={40},
  number={9},
  pages={1643--1646},
  year={2004},
  publisher={Elsevier}
}
@article{jeltsema2003dual,
  title={A dual relation between port-Hamiltonian systems and the Brayton--Moser equations for nonlinear switched RLC circuits},
  author={Jeltsema, Dimitri and Scherpen, Jacquelien MA},
  journal={Automatica},
  volume={39},
  number={6},
  pages={969--979},
  year={2003},
  publisher={Elsevier}
}
@article{venkatraman2010energy,
  title={Energy shaping of port-Hamiltonian systems by using alternate passive input-output pairs},
  author={Venkatraman, Aneesh and van der Schaft, Arjan},
  journal={European Journal of Control},
  volume={16},
  number={6},
  pages={665--677},
  year={2010},
  publisher={Elsevier}
}
@article{ortega2001putting,
  title={Putting energy back in control},
  author={Ortega, Romeo and Van Der Schaft, Arjan J and Mareels, Iven and Maschke, Bernhard},
  journal={IEEE Control Systems},
  volume={21},
  number={2},
  pages={18--33},
  year={2001},
  publisher={IEEE}
}
@book{boyd2004convex,
  title={Convex optimization},
  author={Boyd, Stephen and Vandenberghe, Lieven},
  year={2004},
  publisher={Cambridge university press}
}
@article{brayton1964theory,
  title={A theory of nonlinear networks. I},
  author={Brayton, RK and Moser, JK},
  journal={Quarterly of Applied Mathematics},
  volume={22},
  number={1},
  pages={1--33},
  year={1964}
}
@article{jeltsema2009multidomain,
  title={Multidomain modeling of nonlinear networks and systems},
  author={Jeltsema, Dimitri and Scherpen, Jacquelien MA},
  journal={IEEE Control Systems Magazine},
  volume={29},
  number={4},
  year={2009},
  publisher={IEEE},
  pages={28--59},
}
@article{kelman2013analysis,
  title={Analysis of local optima in predictive control for energy efficient buildings},
  author={Kelman, Anthony and Ma, Yudong and Borrelli, Francesco},
  journal={Journal of Building Performance Simulation},
  volume={6},
  number={3},
  pages={236--255},
  year={2013},
  publisher={Taylor \& Francis}
}
@book{wilcox2008users,
  title={Users manual for TMY3 data sets},
  author={Wilcox, Stephen and Marion, William},
  year={2008},
  publisher={National Renewable Energy Laboratory Golden, CO}
}
@misc{iec,
  author = {ERS},
  title = {{Energy Resource Station Technical Description}},
  howpublished = "\url{http://www.iowaenergycenter.org/energy-resource-station-ers/}",
  year = {2015}  
}
@article{atam2015convex,
  title={A convex approach to a class of non-convex building HVAC control problems: Illustration by two case studies},
  author={Atam, Ercan and Helsen, Lieve},
  journal={Energy and Buildings},
  volume={93},
  pages={269--281},
  year={2015},
  publisher={Elsevier}
}
@article{hovgaard2013nonconvex,
  title={Nonconvex model predictive control for commercial refrigeration},
  author={Hovgaard, Tobias Gybel and Boyd, Stephen and Larsen, Lars FS and J{\o}rgensen, John Bagterp},
  journal={International Journal of Control},
  volume={86},
  number={8},
  pages={1349--1366},
  year={2013},
  publisher={Taylor \& Francis}
}
@article{lavei2011power,
  title={Power flow optimization using positive quadratic programming},
  author={Lavei, Javad and Rantzer, Anders and Low, Stephen},
  journal={IFAC Proceedings Volumes},
  volume={44},
  number={1},
  pages={10481--10486},
  year={2011},
  publisher={Elsevier}
}
@phdthesis{wei2014distributed,
  title={Distributed optimization and market analysis of networked systems},
  author={Wei, Ermin},
  year={2014},
  school={Massachusetts Institute of Technology}
}
@inproceedings{mukherjee2012building,
  title={Building temperature control: A passivity-based approach},
  author={Mukherjee, Sumit and Mishra, Sandipan and Wen, John T},
  booktitle={$\text{51}^{st}$ IEEE Conference on Decision and Control (CDC)},
  pages={6902--6907},
  year={2012}
}
@article{ma2012predictive,
  title={Predictive control for energy efficient buildings with thermal storage: Modeling, stimulation, and experiments},
  author={Ma, Yudong and Kelman, Anthony and Daly, Allan and Borrelli, Francesco},
  journal={IEEE Control Systems},
  volume={32},
  number={1},
  pages={44--64},
  year={2012},
  publisher={IEEE}
}
@inproceedings{deng2010building,
  title={Building thermal model reduction via aggregation of states},
  author={Deng, Kun and Barooah, Prabir and Mehta, Prashant G and Meyn, Sean P},
  booktitle={American Control Conference (ACC), 2010},
  pages={5118--5123},
  year={2010},
  organization={IEEE}
}
@article{ma2012model,
  title={Model predictive control for energy efficient buildings},
  author={Ma, Yudong},
  year={2012}
}
@article{book2011energy,
  title={Energy Efficiency and Renewable Energy},
  author={Book, Buildings Energy Data},
  journal={US department of energy},
  year={2011}
}
@article{ma2016energy,
  title={Energy Management Considering Load Operations and Forecast Errors with Application to HVAC Systems},
  author={Ma, Kai and Hu, Guoqiang and Spanos, Costas J},
  journal={IEEE Transactions on Smart Grid},
  volume={PP},
  number={99},
  pages={1-10},
  year={2016},
  publisher={IEEE}
}

@article{chinde2016building,
  title={A Passivity-Based Power-Shaping Control of Building HVAC Systems},
  author={Chinde, V and Kosaraju, KC and Kelkar, A and Pasumarthy, R and Sarkar, S and Singh, NM},
  journal={Journal of Dynamic Systems, Measurement, and Control},
  volume={139},
  number={11},
  pages={111007--111007-10},
  year={2017},
  publisher={American Society of Mechanical Engineers}
}
@article{stegink2017unifying,
  title={A unifying energy-based approach to stability of power grids with market dynamics},
  author={Stegink, Tjerk and De Persis, Claudio and van der Schaft, Arjan},
  journal={IEEE Transactions on Automatic Control},
  volume={62},
  number={6},
  pages={2612--2622},
  year={2017},
  publisher={IEEE}
}
@article{perez2008review,
	Author = {P{\'e}rez-Lombard, Luis and Ortiz, Jos{\'e} and Pout, Christine},
	Journal = {Energy and buildings},
	Number = {3},
	Pages = {394--398},
	Publisher = {Elsevier},
	Title = {A review on buildings energy consumption information},
	Volume = {40},
	Year = {2008}}
@article{dounis2009advanced,
  title={Advanced control systems engineering for energy and comfort management in a building environment—A review},
  author={Dounis, Anastasios I and Caraiscos, Christos},
  journal={Renewable and Sustainable Energy Reviews},
  volume={13},
  number={6},
  pages={1246--1261},
  year={2009},
  publisher={Elsevier}
}


==> thesis_iitm_intro.tex <==
%\begin{document}
% \chapter{Plan A}
% This chapter copy of iitm file...
\chapter{INTRODUCTION}
\label{chap:intro}

This document provides a simple template of how the provided
\verb+iitmdiss.cls+ \LaTeX\ class is to be used.  Also provided are
several useful tips to do various things that might be of use when you
write your thesis.

Before reading any further please note that you are strongly advised
against changing any of the formatting options used in the class
provided in this directory, unless you are absolutely sure that it
does not violate the IITM formatting guidelines.  \emph{Please do not
  change the margins or the spacing.}  If you do change the formatting
you are on your own (don't blame me if you need to reprint your entire
thesis).  In the case that you do change the formatting despite these
warnings, the least I ask is that you do not redistribute your style
files to your friends (or enemies).

It is also a good idea to take a quick look at the formatting
guidelines.  Your office or advisor should have a copy.  If they
don't, pester them, they really should have the formatting guidelines
readily available somewhere.

To compile your sources run the following from the command line:
\begin{verbatim}
% latex thesis.tex
% bibtex thesis
% latex thesis.tex
% latex thesis.tex
\end{verbatim}
Modify this suitably for your sources.

To generate PDF's with the links from the \verb+hyperref+ package use
the following command:
\begin{verbatim}
% dvipdfm -o thesis.pdf thesis.dvi
\end{verbatim}

\section{Package Options}

Use this thesis as a basic template to format your thesis.  The
\verb+iitmdiss+ class can be used by simply using something like this:
\begin{verbatim}
\documentclass[PhD]{iitmdiss}  
\end{verbatim}

To change the title page for different degrees just change the option
from \verb+PhD+ to one of \verb+MS+, \verb+MTech+ or \verb+BTech+.
The dual degree pages are not supported yet but should be quite easy
to add.  The title page formatting really depends on how large or
small your thesis title is.  Consequently it might require some hand
tuning.  Edit your version of \verb+iitmdiss.cls+ suitably to do this.
I recommend that this be done once your title is final.

To write a synopsis simply use the \verb+synopsis.tex+ file as a
simple template.  The synopsis option turns this on and can be used as
shown below.
\begin{verbatim}
\documentclass[PhD,synopsis]{iitmdiss}                                
\end{verbatim}

Once again the title page may require some small amount of fine
tuning.  This is again easily done by editing the class file.

This sample file uses the \verb+hyperref+ package that makes all
labels and references clickable in both the generated DVI and PDF
files.  These are very useful when reading the document online and do
not affect the output when the files are printed.


\section{Example Figures and tables}

Fig.~\ref{fig:iitm} shows a simple figure for illustration along with
a long caption.  The formatting of the caption text is automatically
single spaced and indented.  Table~\ref{tab:sample} shows a sample
table with the caption placed correctly.  The caption for this should
always be placed before the table as shown in the example.


\begin{figure}[htpb]
  \begin{center}
    \resizebox{50mm}{!} {\includegraphics *{iitm.eps}}
    \resizebox{50mm}{!} {\includegraphics *{iitm.eps}}
    \caption {Two IITM logos in a row.  This is also an
      illustration of a very long figure caption that wraps around two
      two lines.  Notice that the caption is single-spaced.}
  \label{fig:iitm}
  \end{center}
\end{figure}

\begin{table}[htbp]
  \caption{A sample table with a table caption placed
    appropriately. This caption is also very long and is
    single-spaced.  Also notice how the text is aligned.}
  \begin{center}
  \begin{tabular}[c]{|c|r|} \hline
    $x$ & $x^2$ \\ \hline
    1  &  1   \\
    2  &  4  \\
    3  &  9  \\
    4  &  16  \\
    5  &  25  \\
    6  &  36  \\
    7  &  49  \\
    8  &  64  \\ \hline
  \end{tabular}
  \label{tab:sample}
  \end{center}
\end{table}

\section{Bibliography with BIB\TeX}

I strongly recommend that you use BIB\TeX\ to automatically generate
your bibliography.  It makes managing your references much easier.  It
is an excellent way to organize your references and reuse them.  You
can use one set of entries for your references and cite them in your
thesis, papers and reports.  If you haven't used it anytime before
please invest some time learning how to use it.  

I've included a simple example BIB\TeX\ file along in this directory
called \verb+refs.bib+.  The \verb+iitmdiss.cls+ class package which
is used in this thesis and for the synopsis uses the \verb+natbib+
package to format the references along with a customized bibliography
style provided as the \verb+iitm.bst+ file in the directory containing
\verb+thesis.tex+.  Documentation for the \verb+natbib+ package should
be available in your distribution of \LaTeX.  Basically, to cite the
author along with the author name and year use \verb+\cite{key}+ where
\verb+key+ is the citation key for your bibliography entry.  You can
also use \verb+\citet{key}+ to get the same effect.  To make the
citation without the author name in the main text but inside the
parenthesis use \verb+\citep{key}+.  The following paragraph shows how
citations can be used in text effectively.

More information on BIB\TeX\ is available in the book by
\cite{lamport:86}.  There are many
references~\citep{lamport:86,prabhu:xx} that explain how to use
BIB\TeX.  Read the \verb+natbib+ package documentation for more
details on how to cite things differently.

Here are other references for example.  \citet{viz:mayavi} presents a
Python based visualization system called MayaVi in a conference paper.
\citet{pan:pr:flat-fst} illustrates a journal article with multiple
authors.  Python~\citep{py:python} is a programming language and is
cited here to show how to cite something that is best identified with
a URL.

\section{Other useful \LaTeX\ packages}

The following packages might be useful when writing your thesis.

\begin{itemize}  
\item It is very useful to include line numbers in your document.
  That way, it is very easy for people to suggest corrections to your
  text.  I recommend the use of the \texttt{lineno} package for this
  purpose.  This is not a standard package but can be obtained on the
  internet.  The directory containing this file should contain a
  lineno directory that includes the package along with documentation
  for it.

\item The \texttt{listings} package should be available with your
  distribution of \LaTeX.  This package is very useful when one needs
  to list source code or pseudo-code.

\item For special figure captions the \texttt{ccaption} package may be
  useful.  This is specially useful if one has a figure that spans
  more than two pages and you need to use the same figure number.

\item The notation page can be entered manually or automatically
  generated using the \texttt{nomencl} package.

\end{itemize}

More details on how to use these specific packages are available along
with the documentation of the respective packages.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\end{document}
